EGG-GAE: scalable graph neural networks for tabular data imputation

Missing data imputation (MDI) is crucial when dealing with tabular datasets across various domains. Autoencoders can be trained to reconstruct missing values, and graph autoencoders (GAE) can additionally consider similar patterns in the dataset when imputing new values for a given instance. However, previously proposed GAEs suffer from scalability issues, requiring the user to define a similarity metric among patterns to build the graph connectivity beforehand. In this paper, we leverage recent progress in latent graph imputation to propose a novel EdGe Generation Graph AutoEncoder (EGG-GAE) for missing data imputation that overcomes these two drawbacks. EGG-GAE works on randomly sampled mini-batches of the input data (hence scaling to larger datasets), and it automatically infers the best connectivity across the mini-batch for each architecture layer. We also experiment with several extensions, including an ensemble strategy for inference and the inclusion of what we call prototype nodes, obtaining significant improvements, both in terms of imputation error and final downstream accuracy, across multiple benchmarks and baselines.

==> experiments/ensembling_exp.tex <==
\subsubsection{Ensembling experiment}
\label{ensembling_experiment}

In this section we investigate the changes of the downstream task score (end-to-end accuracy) along with imputation prediction performance (RMSE and MAE) by varying  the number of ensembling iterations in $\left\{1, 5, 10, 20, 50\right\}$. Figure \ref{ensemble_average_ranking} shows that performing ensembling during inference enhances the performance of downstream and MDI problems regardless of missingness mechanisms. We can see that an increasing number of ensembling iterations on average cause the improvement for every type of missingness, as hypothesized. Both EGG-GAE-20 and EGG-GAE-50 have close mean values, while the corresponding variations share the same interval (around $[1.3, 2.8]$); this indicates that the plateau is achieved when increasing the number of iterations to more than 20. We argue that performing ensembling during the inference leads to (i) reliable performance (ii) enhancing the performance of downstream and MDI problems.

\begin{figure}[t]
    \centerline{\includegraphics[width=0.9\columnwidth]{images/unified_AR_ens.png}}
    \caption{Unified average ranking computed for the MCAR, MNAR, and MAR scenarios.  A value following the model name indicates the number of ensembling iterations.}
    \label{ensemble_average_ranking}
\end{figure}


==> experiments/proto_exp.tex <==
\subsubsection{Prototype node evaluation} 
\label{proto_sec.}

This section investigates the effect of the introduced learnable prototype nodes.Figure \ref{proto_average_ranking} shows that the models with learnable prototype nodes (EGG-GAE-10, EGG-GAE-20, EGG-GAE-50) have a lower mean average ranking compared to the model without them (EGG-GAE-0), independent of the missingness mechanisms scenario. Increasing the number of prototype nodes helps to achieve better performance. However, we can see that introducing a significant number of prototype nodes might worsen the performance (EGG-GAE-50). We believe that  that the number of prototype nodes should be at least equal to the number of classes of downstream tasks. However, adding too many of prototype nodes can impair the performance. We believe it affects the sampling scheme by increasing the likelihood that the graphs will be built primarily with prototype nodes, resulting in a poorer solution.

\begin{figure*}[!ht]
  \centering
  \begin{subfigure}[b]{0.45\linewidth}
    \centerline{\includegraphics[width=\textwidth]{images/unified_AR_ens.png}}
    \caption{prototype nodes}
    \label{ensemble_average_ranking}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\linewidth}
    \centerline{\includegraphics[width=\textwidth]{images/unified_AR_proto.png}}
    \caption{Ensembling}
    \label{proto_average_ranking}
  \end{subfigure}
  \caption{Unified average ranking computed for the MCAR, MNAR, and MAR scenarios.  A value following the model name represents the variable parameter.}
  \label{fig:unified_plots}
\end{figure*}

% \begin{figure}[t]
%     \centerline{\includegraphics[width=0.9\columnwidth]{images/unified_AR_proto.png}}
%      \caption{Unified average ranking computed for the MCAR, MNAR, and MAR scenarios. A value following the model name indicates the number of prototype nodes.}
%     \label{proto_average_ranking}
% \end{figure}









==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
